Kernel Methods are Competitive for Operator Learning

We present a general kernel-based framework for learning operators between Banach spaces along with a priori error analysis and comprehensive numerical comparisons with popular neural net (NN) approaches such as Deep Operator Net (DeepONet) [Lu et al.] and Fourier Neural Operator (FNO) [Li et al.]. We consider the setting where the input/output spaces of target operator $\mathcal{G}^\dagger\,:\, \mathcal{U}\to \mathcal{V}$ are reproducing kernel Hilbert spaces (RKHS), the data comes in the form of partial observations $\phi(u_i), \varphi(v_i)$ of input/output functions $v_i=\mathcal{G}^\dagger(u_i)$ ($i=1,\ldots,N$), and the measurement operators $\phi\,:\, \mathcal{U}\to \mathbb{R}^n$ and $\varphi\,:\, \mathcal{V} \to \mathbb{R}^m$ are linear. Writing $\psi\,:\, \mathbb{R}^n \to \mathcal{U}$ and $\chi\,:\, \mathbb{R}^m \to \mathcal{V}$ for the optimal recovery maps associated with $\phi$ and $\varphi$, we approximate $\mathcal{G}^\dagger$ with $\bar{\mathcal{G}}=\chi \circ \bar{f} \circ \phi$ where $\bar{f}$ is an optimal recovery approximation of $f^\dagger:=\varphi \circ \mathcal{G}^\dagger \circ \psi\,:\,\mathbb{R}^n \to \mathbb{R}^m$. We show that, even when using vanilla kernels (e.g., linear or Mat\'{e}rn), our approach is competitive in terms of cost-accuracy trade-off and either matches or beats the performance of NN methods on a majority of benchmarks. Additionally, our framework offers several advantages inherited from kernel methods: simplicity, interpretability, convergence guarantees, a priori error estimates, and Bayesian uncertainty quantification. As such, it can serve as a natural benchmark for operator learning.

==> stuff.tex <==
\newpage
\section{Stuff}


\section{Outstanding work}

Elements I would like to be introduced:

\begin{enumerate}
    \item Theoretical guarantees of kernel regression. The universal approximation property seems important.
    \item Add the results comparing with the cost-accuracy paper.
    \item Add discussion on complexity.
    \item Add discussion on uncertainty quantification with GPs - done.
    \item Mention the size of datasets.
\end{enumerate}


\section{Introduction}
\md{This section should feature a brief description of operator learning and its application, emphasizing the role of surrogate modeling and many-query motivation.}



The approximation of solutions in the context of Partial Differential Equations (PDEs) has long relied on expensive, but accurate numerical solvers. Data-driven methods have recently found success in learning operators between function spaces. Once trained, approximate operators learned from data are effective surrogates for traditional solvers, enabling the fast computation of solution of PDEs with minimal loss in accuracy. These surrogates are particularly effective when the solution needs to be evaluated many times, such as in the context of monte carlo simulations or PDE-constrained optimization.
The most popular methods for learning operators from data are based on neural networks. Two major examples are the Deep Operator Net (DeepONet) and the Fourier Neural Operators (FNO). In this paper, we will examine an alternative to neural networks, based on the classical machine learning method of kernels. We will show that kernel methods provide a simple and interpretable alternative to neural networks which is competitive in the cost accuracy tradeoff. We will compare the performance on several benchmarks present in the literature and present some initial theoretical results on their convergence. Moreover we will critically examine some of the benchmarks present in the literature and asses their suitability. The goal of this paper is threefold:
\begin{enumerate}
    \item To show that kernel methods are competitive with neural operators for operator learning and provide a general framework for their application to these tasks.
    \item To show that certain problems considered in the literature are too simple to be effective benchmarks and to steer researchers toward more challenging problems.
    \item To show that classical machine learning methods perform well in the context of operator learning with minimal modifications.
\end{enumerate}

\subsection{Why kernel methods?} \md{I am not too sure how to format this but I would like a small paragraph that explains at a high level why we should consider kernel methods} \pb{Andrew paper has lots of references in the introduction, include them}
Kernel methods have long been known to be effective for the regression and interpolation of a scalar-valued function $f: \mathbb{R}^d \to \mathbb{R}$. They have been extended to provide effective solutions of non-linear PDEs  \cite{gp_pdes} \md{insert applications in CSE here/references}. Kernel methods present several distinct advantages
\begin{itemize}
    \item Solving regression problems reduces to solving a linear system, without the need for gradient descent or backpropagation (Section \ref{sec: kernel regression for operators}).
    \item Their theoretical simplicity allows to easily obtain theoretical guarantees (Section \ref{sec: theoretical guaranteess}).
    \item Their interpretation as the conditioning of a Gaussian Process automatically yields uncertainty quantification bounds.
    \item Empirically, a very simple kernel method is competitive with operator neural networks in the cost-accuracy tradeoff (Section \ref{sec: Numerical results}).
\end{itemize}
These virtues can be easily transferred to the setting of operator learning. Moreover, our experiments show that, empirically, a very simple kernel method is competitive with operator neural networks in the cost-accuracy tradeoff (Section \ref{sec: Numerical results}), therefore opening up new research directions in this area.
\section{Operator Learning}
In this section, we present the general formulation of operator learning and present general formulations for problems that arise from Partial Differential Equations.
\subsection{Problem formulation}\label{subsec:notation}
We follow the setting of \cite{cost_accuracy}. Consider two Banach spaces of functions $\mathcal{U}$ and $\mathcal{V}$:
\begin{align}
        &\mathcal{U} = \{ u: D_u \to \mathbb{R}^{d_i} \}, \quad D_u \subseteq \mathbb{R}^{d_x} \\
         &\mathcal{V} = \{ v: D_v \to \mathbb{R}^{d_0} \}, \quad D_v \subseteq \mathbb{R}^{d_y}.
\end{align}
 We aim learn an arbitrary operator $\mathcal{G} :\mathcal{U} \to \mathcal{V}$ from data pairs $\{u_i, v_i\}_{i = 1}^N$, where $u_i$ are i.i.d samples from a measure $\mu$ supported on $\mathcal{U}$ and
\begin{equation}
        \mathcal{G}(u_i) = v_i, \quad \text{for } i =1, \dots, N.
\end{equation}
Therefore, Note the problem depends both on $\mathcal G$ (in the examples coming from PDEs, the type of problem considered and particular equation) and $\mu$ (in the examples coming from PDEs, the distribution from which the dataset, usually obtained with traditional numerical methods, is sample). We emphasize this fact because, notably, the difficulty of an operator learning problem depends on the distribution $\mu$; a highly complicated operator $\mathcal G$ might be close to linear (or even constant)in the support of a particular $\mu$. We will illustrate this fact with our numerical results, which show that for an example coming from the advection equation, keeping $\mathcal G$ constant but varying $\mu$ leads to vastly different performance consistently across all methods benchmarked.
\subsection{Evaluation metrics}
\md{This section should introduce the metrics we use to measure performance: the relative $L^2$ loss and the cost-accuracy tradeoff.}
As was convincingly argued in \cite{cost_accuracy}, given that surrogate models aim to emulate exact models for a fraction of the cost and with minimal loss in accuracy, operator learning methods should be evaluated in the cost-accuracy tradeoff. Depending on the application, a gain in accuracy may not be worth the added complexity required by the model. Similarly, understanding how models scale in accuracy in terms of complexity is key to evaluating the best method for a given application. \pb{Can we think of convincing examples that illustrate this point?} Here we present the metrics used to measure both the accuracy and the complexity of the model.
\subsubsection{Measure of accuracy}
To measure the performance we evaluate the accuracy of our models as measured by a relative loss on the space of output functions $\mathcal V$ .
\begin{equation}
    \mathcal{R}(\mathcal{G}) = \mathbb{E}_{u \sim \mu} \Bigg[\frac{\norm{\mathcal{G}(u) - \mathcal{G}^{\dagger}(u)}_{\mathcal V}}{\norm{\mathcal{G}(u)}_{\mathcal V}} \Bigg]
\end{equation}
where $\mathcal{G}$ is true operator and $\mathcal{G}^\dagger$ is our recovery of the operator from data. Following previous work, $\norm{u}_{\mathcal V} = \norm{u}_{L^2} := (\int u(x)^2dx)^{\frac{1}{2}}$ is usually taken, and it is computed from pointwise measurements with the trapezoidal rule. In practice, we do not have the access to the underlying probability measure $\mu$ and we compute the empirical loss on a withheld test set:
\begin{equation}\label{eq:loss}
    \mathcal{R}_N(\mathcal{G}) = \frac{1}{N} \sum_{i=1}^N \Bigg[\frac{\norm{\mathcal{G}(u_i) - \mathcal{G}^{\dagger}(u_i)}_{\mathcal V}}{\norm{\mathcal{G}(u_i)}_{\mathcal V}} \Bigg]
\end{equation}

\subsubsection{Measure of complexity}\label{subsec:complex}
\paragraph{Training complexity}
Even though the online evaluation complexity eventually dominates the cost of training, the computational resources that can be allocated in different settings and applications are not always large; therefore numerical methods in which the offline data assimilation step is cheaper, faster, and more robust will always be preferred. Computing the exact number of FLOPs at training time is very hard to do a priori for neural network methods, as it depends on the optimization algorithm used, the hyperparameters and the optimization over such hyperparameters, among others. Therefore in this work we limit the training complexity evaluation to be purely qualitative. Nevertheless, all the methods provided in this work are significantly simpler at training time, as they have no neural network weights, few or no hyperparameters to tune, and the tuning of such can be done, among others, by one run of gradient descent.

\paragraph{Inference complexity}
Complexity at inference time is the main metric used in \cite{cost_accuracy} to compare numerical methods for operator learning. The motivation is that training of the methods can be performed in an offline fashion, and therefore the cost per test example dominates in the limit of many test queries. In particular, they compare the online evaluation costs of the neural networks by computing the requisite floating point operations (FLOPs) per test example. We adopt this metric as well for the methods not based on neural networks that we develop in this work, and we compare, when available, the cost-accuracy tradeoff with the numbers reported in \cite{cost_accuracy}

\subsection{Example problems arising from PDEs} \label{subsec:exampleproblems}
We now present abstract formulations of canonical operator learning problems arising in the context of PDEs. While this list is not exhaustive, the aim of this section is to place our numerical experiments within the larger context of operator learning for PDEs. For each problem, we indicate the numerical experiment that corresponds to the problem.

\subsubsection{Solution operator}
Consider the (possibly non-linear) PDE of order $n$:
\begin{subequations} \label{eq:solution_operator}
    \begin{align}
        \mathcal{P}(D^nu, D^{n-1}u, \dots, u, x) &= f \quad x \in \Omega \\
        \mathcal{B}(D^nu, D^{n-1}u, \dots, u, x) &= 0 \quad x \in \partial\Omega.
    \end{align}
\end{subequations}
In this case, $\mathcal{G}$ is the solution operator mapping the forcing term to the solution
\begin{equation}
    \mathcal{G}: f \mapsto u
\end{equation}
Examples include the forced Navier-Stokes equations in  2 and 3 dimensions in Section \ref{sec: navier stokes}.
\subsubsection{Boundary value problem}
Consider the general form of a time-dependent PDE:
\begin{subequations} \label{eq:bvp}
    \begin{align}
        \partial_t u + \mathcal{P}(D^nu, D^{n-1}u, \dots, u, x) &= 0 \quad (t,x) \in \mathbb{R}^{+} \times \Omega\\
        u(t, x) &= f \quad (t,x) \in \mathbb{R}^{+} \times \partial \Omega \\
        u(0, x) &= g \quad x \in \Omega.
    \end{align}
\end{subequations}
The operator $\mathcal{G}$ maps the initial condition to the solution at time $T$ (for time-dependent problems) or the value at the boundary to the solution (for time-independent problems):
\begin{align}
    &\mathcal{G}: u(0, x) \mapsto u(T,x) \\
    &\mathcal{G}: f \mapsto u(x).
\end{align}
Examples include Burgers's equation in Section \ref{sec: burger}, and the Advection equation in Sections \ref{sec: advection 1}. The structural mechanics equation in Section \ref{sec: structural eq} is an example of a time-independent boundary value problem.

\subsubsection{Inverse problem (parametric)}
 Consider a PDE dependent on a coefficient $a$ given by
 \begin{subequations} \label{eq:IP}
    \begin{align}
        \mathcal{P}(D^nu, D^{n-1}u, \dots, u, x; a) &= f \quad x \in \Omega \\
        \mathcal{B}(D^nu, D^{n-1}u, \dots, u, x) &= 0 \quad x \in \partial\Omega.
    \end{align}
\end{subequations}

For a fixed forcing term $f$, the inverse problem is to learn the map
\begin{equation}
    \mathcal{G}: a \mapsto u.
\end{equation}
Examples include the Darcy flow problem in Section \ref{sec: darcy problem} and Helmholtz equation in Section \ref{sec: helmholtz}.


\appendix

\section{Expressions for the kernels used in experiments}\label{app: kernels}
The following can be found in many standard textbooks on Gaussian processes such as \cite{rasmussen}.
\paragraph{The Mat\'{e}rn parametric family}
Let $r = \norm{\bold{u}_1 - \bold{u}_2}$.  For $\nu = p + \frac{1}{2}, p \in \mathbb{Z}_{+}$, the Mat\'{e}rn covariance can be written as:
\begin{equation}
    K_{\nu =p + \frac{1}{2}}(r) = \exp\bigg(-\frac{\sqrt{2\nu} r}{l}\bigg)\frac{\Gamma(p+1)}{\Gamma(2p+1)}\sum_{i=0}^p \frac{(p+1)!}{i!(p-i)!}\bigg( \frac{\sqrt{8\nu}r}{l}\bigg)^{p-i}
\end{equation}
In the limiting case where $\nu \to \infty$, the Mat\'{e}rn kernel, we obtain the Gaussian or squared exponential kernel:
\begin{equation}
    k_{\nu = \infty}(r) = \exp\bigg(-\frac{r^2}{2l^2}\bigg).
\end{equation}
\paragraph{The inverse quadratic kernel} The inverse quadratic kernel has the expression
\begin{equation}
    k_{\text{RQ}} = \bigg( 1+ \frac{r^2}{2 l^2} \bigg)^{-\alpha}.
\end{equation}

\section{The Gaussian Process interpretation}

We briefly present the Gaussian process perspective on kernel methods. This material here is presented in greater detail with a proof of the theorem in \cite{plato_shapes}. The key takeaway from this section is that fitting a kernel method to an interpolation problem can be interpreted as conditioning a Gaussian process with zero mean. The Gaussian process conditional covariance can then be used to provide uncertainty quantification.

We first extend the notion of Gaussian Processes to operator-valued Gaussian processes.
\begin{definition}
Let $k: \mathcal{X} \times \mathcal{X} \rightarrow \mathcal{L}(\mathcal{Y})$ be an operator-valued kernel as in Sec. \ref{sec: operator valued kernels}. Let $m$ be a function mapping $\mathcal{X}$ to $\mathcal{Y}$. We call $\xi\,:\, \mathcal{X} \rightarrow  \mathcal{L}(\mathcal{Y}, {\bf H})$ a operator-valued Gaussian process if
 $\xi$ is a function mapping
$x \in \mathcal{X}$ to $\xi(x)\in \mathcal{L}(\mathcal{Y},{\bf H})$ where ${\bf H}$ is a Gaussian space\footnote{That is a Hilbert space of centered Gaussian random variables, see \cite[Sec.~7\&17]{owhadi_scovel_2019}.} and $ \mathcal{L}(\mathcal{Y}, {\bf H})$ is the space of bounded linear operators $\mathcal{Y}$ to ${\bf H}$. Abusing notations we write $\langle\xi(x),y\rangle_\mathcal{Y}$ for $\xi(x)y$. We say that $\xi$ has mean $m$ and covariance kernel $K$ and write $\xi \sim \mathcal{N}(m,K)$ if $\langle\xi(x),y\rangle_{\mathcal{Y}} \sim \mathcal{N}\big(m(x),y^T K(x,x)y\big)$ and
\begin{equation}
\text{Cov}\big(\langle\xi(x),y\rangle_{\mathcal{Y}}, \langle\xi(x'),y'\rangle_{\mathcal{Y}}\big)=y^T K(x,x')y'\,.
\end{equation}
We say that $\xi$ is centered if it is of zero mean.
\end{definition}

The next proposition identifies the kernel regression solution with kernel $k$ with the conditional mean of the Gaussian process with a covariance defined by $k$ and provides .
\begin{theorem}
Let $\xi$ be a centered operator-valued GP with covariance kernel $ \mathcal{X} \times \mathcal{X} \rightarrow \mathcal{L}(\mathcal{Y})$. Let $X,Y\in \mathcal{X}^N\times \mathcal{Y}^N$.Then $\xi$ conditioned on $\xi(X)$ is a operator-valued GP with mean
\begin{equation}\label{eq: conditional mean}
\E\big[\xi(x)\big| \xi(X)=Y\big]=K(x,X)\big(K(X,X)\big)^{-1} Y
\end{equation}
and conditional covariance operator
\begin{equation}\label{eq: conditional cov}
K^\perp(x,x'):=K(x,x')-K(x,X)\big(K(X,X)\big)^{-1}K(X,x')\,.
\end{equation}
In particular, if $k$ is trace class, then
\begin{equation}\label{eq: conditional var}
\sigma^2(x):=\E\Big[\big\|\xi(x) -\E[\xi(x)| \xi(X)=Y]\big\|_{\mathcal{Y}}^2\Big| \xi(X)=Y\Big] = \textrm{Tr}\big[K^\perp(x,x)\big]\,.
\end{equation}
\end{theorem}
Observe that equation \eqref{eq: conditional mean} shows that the conditional mean of $\xi$ provides the same solution as that given by the kernel regression solution \eqref{eq: optimal recov expression}. Moreover equations \eqref{eq: conditional cov} and \eqref{eq: conditional var} provide uncertainty quantification for the prediction of new data point.

The quantity $\sigma$ also provides deterministic error bounds on the kernel regression solution.

\begin{theorem}[Deterministic error bounds]
    Let $\mathcal{F}^*$ be the true solution to the problem \eqref{eq: functional regression prob} and let $\mathcal{F}^{\dagger}$ be the solution defined by Theorem \ref{thm: represented theorem}. Then
    \begin{equation}
        \norm{\mathcal{F}^{\dagger}(x) - \mathcal{F}^{*}(x)}_{\mathcal{Y}}^2 \leq \sigma(x)\norm{\mathcal{F}^{*}}_{\mathcal{H}}^2.
    \end{equation}
\end{theorem}

\begin{remark}
    Note that in the infinite measurement limit (i.e. as the measurement function $\varphi$ recover the value of $v$ in the entire domain), our choice of kernel \eqref{eq: kernel times identity} yields the identity which is not a trace class operator and hence the above error bounds cannot be applied. However one can note that for any set of \textit{finite} measurements, our operator-valued kernel is trace class and therefore yields valid error bounds.  If one wishes to consider trace class operators in the infinite measurement limit, a possible choice is that defined by \cite{kadri_kernels}:
    \begin{equation}
        K(\bold{u}_1,\bold{u_2}) = G(\bold{u}_1,\bold{u_2})T
    \end{equation}
    where $G$ is a scalar-valued kernel and $T$ is some trace class operator on $\mathcal{V}$.
    \end{remark}

